Statistical Rejection Sampling Improves Preference Optimization

Improving the alignment of language models with human preferences remains an active research challenge. Previous approaches have primarily utilized Reinforcement Learning from Human Feedback (RLHF) via online RL methods such as Proximal Policy Optimization (PPO). Recently, offline methods such as Sequence Likelihood Calibration (SLiC) and Direct Preference Optimization (DPO) have emerged as attractive alternatives, offering improvements in stability and scalability while maintaining competitive performance. SLiC refines its loss function using sequence pairs sampled from a supervised fine-tuned (SFT) policy, while DPO directly optimizes language models based on preference data, foregoing the need for a separate reward model. However, the maximum likelihood estimator (MLE) of the target optimal policy requires labeled preference pairs sampled from that policy. DPO's lack of a reward model constrains its ability to sample preference pairs from the optimal policy, and SLiC is restricted to sampling preference pairs only from the SFT policy. To address these limitations, we introduce a novel approach called Statistical Rejection Sampling Optimization (RSO) that aims to source preference data from the target optimal policy using rejection sampling, enabling a more accurate estimation of the optimal policy. We also propose a unified framework that enhances the loss functions used in both SLiC and DPO from a preference modeling standpoint. Through extensive experiments across three diverse tasks, we demonstrate that RSO consistently outperforms both SLiC and DPO on evaluations from both Large Language Model (LLM) and human raters.

==> tables/main_results.tex <==
\begin{table}[h]\small
\begin{center}
\begin{tabular}{lllcc}
\hline
Approach & \multicolumn{2}{c}{ Ablation}  &  \multicolumn{2}{c}{ Metrics } \\
 &   Loss & Preference Pair & Reward Model (\%) & AutoSxS (\%) \tablefootnote{The numbers are lower than Reward Model win rate because AutoSxS has three classes: A, B, or Same, while Reward Model only has two classes A or B. Besides, AutoSxS scores have lower risk of reward hacking.}%& Relative Length
\\ 
\hline\hline
\multicolumn{5}{c}{\textbf{Reddit TL;DR}}\\
\hline
 DPO  & sigmoid-norm & direct          & 84.35 & 67.72 \\ %& 1.45 \\
      & sigmoid-norm & sft-sample-rank & 88.63 & 69.02 \\ %& 1.32 \\
 $\text{RSO}_\text{sigmoid-norm}$ & sigmoid-norm & rso-sample-rank & \textbf{92.37} & \textbf{71.86} \\ %& 1.50 \\
 $\text{SLiC}_\text{direct}$ & hinge        & direct          & 86.92 & 60.54 \\ %& 1.78 \\
 $\text{SLiC}_\text{sample-rank}$ & hinge        & sft-sample-rank & 89.75 & 67.04 \\ %& 1.41  \\
      & hinge        & rso-sample-rank & \textbf{93.36} & \textbf{69.26} \\ %& 1.56   \\
      & hinge-norm   & direct          & 83.93 & 66.63 \\ %& 1.39 \\
      & hinge-norm   & sft-sample-rank & 88.04 & 68.46 \\ %& 1.33 \\
 $\text{RSO}_\text{hinge-norm}$ & hinge-norm   & rso-sample-rank & \textbf{92.80} & \textbf{70.84} \\ %& 1.51  \\
\hline
\hline
\multicolumn{5}{c}{\textbf{CNN/DailyMail}}\\
\hline
 DPO  & sigmoid-norm & direct          & 61.31 & 37.36 \\ %& 0.80  \\
      & sigmoid-norm & sft-sample-rank & 62.72 & 38.63 \\ %& 0.60  \\
 $\text{RSO}_\text{sigmoid-norm}$ & sigmoid-norm & rso-sample-rank & \textbf{69.38} & \textbf{39.71} \\ %& 0.96 \\
 $\text{SLiC}_\text{direct}$ & hinge        & direct          & 64.18 & 33.63 \\ %& 0.96 \\
 $\text{SLiC}_\text{sample-rank}$ & hinge        & sft-sample-rank & 67.16 & 33.21 \\ %& 0.93 \\
      & hinge        & rso-sample-rank & \textbf{71.62} & \textbf{35.46} \\ %& 1.10   \\
      & hinge-norm   & direct          & 60.04 & 33.91 \\ %& 0.76 \\
      & hinge-norm   & sft-sample-rank & 61.77 & 40.63 \\ %& 0.60 \\
 $\text{RSO}_\text{hinge-norm}$ & hinge-norm   & rso-sample-rank & \textbf{69.82} & \textbf{42.18} \\ %& 1.02 \\
\hline\hline
\multicolumn{5}{c}{\textbf{AnthropicHH}}\\
\hline
 DPO  & sigmoid-norm & direct          & 51.63 & 24.01 \\ %& 2.34  \\
      & sigmoid-norm & sft-sample-rank & 85.09 & 39.56 \\ %& 1.94  \\
 $\text{RSO}_\text{sigmoid-norm}$ & sigmoid-norm & rso-sample-rank & \textbf{86.94} & \textbf{40.98} \\ %& 2.37  \\
 $\text{SLiC}_\text{direct}$ & hinge        & direct          & 35.95 & 15.69  \\
 $\text{SLiC}_\text{sample-rank}$ & hinge        & sft-sample-rank & 80.82 & 30.66 \\
      & hinge        & rso-sample-rank & \textbf{82.21} & \textbf{32.56} \\
      & hinge-norm   & direct          & 49.55 & 22.89  \\
      & hinge-norm   & sft-sample-rank & 82.40 & 35.96  \\
 $\text{RSO}_\text{hinge-norm}$ & hinge-norm   & rso-sample-rank & \textbf{84.44} & \textbf{38.58} \\
\hline
\end{tabular}
\caption{Compare different methods to leverage human feedback data on three tasks. ``direct'' preference pair directly comes from human preference data. ``sft-sample-rank'' preference pair uses SFT policy to sample 4 pairs for each training example input text and get them labeled by the pairwise reward model. ``rso-sample-rank'' preference pair uses rejection sampling to sample 4 pairs for each training example input text and get them labeled by the pairwise reward model. Both pairwise reward model and few-shot PaLM 2-L win rate against SFT target text are reported. RSO shows improvement on three tasks over DPO and SLiC with a clear margin.}
\label{tab:main_results}
\end{center}

\end{table}


